Learning Simple Algorithms from Examples

We present an approach for learning simple algorithms such as copying, multi-digit addition and single digit multiplication directly from examples. Our framework consists of a set of interfaces, accessed by a controller. Typical interfaces are 1-D tapes or 2-D grids that hold the input and output data. For the controller, we explore a range of neural network-based models which vary in their ability to abstract the underlying algorithm from training instances and generalize to test examples with many thousands of digits. The controller is trained using $Q$-learning with several enhancements and we show that the bottleneck is in the capabilities of the controller rather than in the search incurred by $Q$-learning.

==> Makefile <==
PARTS=main.tex

all: clean main.pdf 

main.pdf: $(PARTS) bibliography.bib 
	pdflatex -shell-escape main.tex
	bibtex main
	bibtex main
	pdflatex -shell-escape main.tex
	pdflatex -shell-escape main.tex

clean:
	rm -f *.log *.blg *.aux *.bbl *.4tc *.xref *.tmp *.dvi *.hd *.idx *.out *.toc *.drv *.ins *.py *.pdf
	rm -rf ~*
	rm -rf *.tmp
	rm -rf *.4om
	rm -rf *~

tar:
	find . -type f | egrep -v '\.git|\.log|\.swp' | xargs tar zcvf ../inter.tar.gz


==> experiments/table_base.tex <==
\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|lccccccccc|}
\hline 
\multicolumn{1}{|l|}{\backslashbox{Task}{Vocabulary Size}} & \multicolumn{1}{|c|}{2} & \multicolumn{1}{|c|}{3} & \multicolumn{1}{|c|}{4} & \multicolumn{1}{|c|}{5} & \multicolumn{1}{|c|}{6} & \multicolumn{1}{|c|}{7} & \multicolumn{1}{|c|}{8} & \multicolumn{1}{|c|}{9} & \multicolumn{1}{|c|}{10}\\\hline 
Coping & \cellcolor{color_10_6!25} 1.4 & \cellcolor{color_10_4!25} 0.6 & \cellcolor{color_10_4!25} 0.6 & \cellcolor{color_10_4!25} 0.6 & \cellcolor{color_10_4!25} 0.6 & \cellcolor{color_10_4!25} 0.5 & \cellcolor{color_10_4!25} 0.6 & \cellcolor{color_10_4!25} 0.6 & \cellcolor{color_10_4!25} 0.6\\
Reverse & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0\\
Reverse & \cellcolor{color_10_5!25} 6.5 & \cellcolor{color_10_10!25} 23.8 & \cellcolor{color_10_4!25} 3.1 & \cellcolor{color_10_4!25} 3.6 & \cellcolor{color_10_4!25} 3.8 & \cellcolor{color_10_4!25} 2.5 & \cellcolor{color_10_4!25} 2.8 & \cellcolor{color_10_3!25} 2.0 & \cellcolor{color_10_4!25} 3.1\\
Walk & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0\\
Walk (FF) & \cellcolor{color_10_10!25} 250.0 & \cellcolor{color_10_3!25} 37.7 & \cellcolor{color_10_4!25} 46.7 & \cellcolor{color_10_3!25} 36.2 & \cellcolor{color_10_3!25} 14.4 & \cellcolor{color_10_3!25} 16.9 & \cellcolor{color_10_3!25} 21.3 & \cellcolor{color_10_3!25} 15.1 & \cellcolor{color_10_10!25} 250.0\\
walk3 & \cellcolor{color_10_10!25} 250.0 & \cellcolor{color_10_2!25} 21.6 & \cellcolor{color_10_2!25} 11.9 & \cellcolor{color_10_3!25} 47.1 & \cellcolor{color_10_7!25} 164.7 & \cellcolor{color_10_10!25} 250.0 & \cellcolor{color_10_6!25} 135.8 & \cellcolor{color_10_2!25} 19.8 & \cellcolor{color_10_1!25} 7.5\\
walk3_ff & \cellcolor{color_10_7!25} 8.7 & \cellcolor{color_10_5!25} 6.9 & \cellcolor{color_10_5!25} 6.8 & \cellcolor{color_10_2!25} 4.0 & \cellcolor{color_10_4!25} 6.2 & \cellcolor{color_10_3!25} 5.3 & \cellcolor{color_10_2!25} 4.4 & \cellcolor{color_10_2!25} 3.9 & \cellcolor{color_10_10!25} 11.1\\
Addition & \cellcolor{color_10_10!25} 250.0 & \cellcolor{color_10_4!25} 30.9 & \cellcolor{color_10_4!25} 14.5 & \cellcolor{color_10_4!25} 26.1 & \cellcolor{color_10_4!25} 21.8 & \cellcolor{color_10_4!25} 21.9 & \cellcolor{color_10_4!25} 25.0 & \cellcolor{color_10_4!25} 23.4 & \cellcolor{color_10_4!25} 21.1\\
3-number Addition & \cellcolor{color_10_10!25} 250.0 & \cellcolor{color_10_0!25} 61.5 & \cellcolor{color_10_10!25} 250.0 & \cellcolor{color_10_10!25} 250.0 & \cellcolor{color_10_3!25} 112.2 & \cellcolor{color_10_6!25} 178.2 & \cellcolor{color_10_2!25} 93.8 & \cellcolor{color_10_1!25} 79.1 & \cellcolor{color_10_1!25} 81.9\\
Single Digit Multiplication & invalid & \cellcolor{color_10_0!25} 6.2 & \cellcolor{color_10_4!25} 17.8 & \cellcolor{color_10_5!25} 20.9 & \cellcolor{color_10_5!25} 21.4 & \cellcolor{color_10_5!25} 21.5 & \cellcolor{color_10_6!25} 22.3 & \cellcolor{color_10_6!25} 23.3 & \cellcolor{color_10_7!25} 24.7\\
\hline 


==> experiments/table_contrastive.tex <==
\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|l|cc|cc|}
\hline 
 \multicolumn{1}{|l|}{\backslashbox{Task}{Penalty on $Q(s, \bullet)$}}  & No decay & Decay & No decay & Decay \\
\hline 
 & \multicolumn{2}{c|}{Test complexity = 100} & \multicolumn{2}{c|}{Test complexity = 10000} \\
\hline 
Coping & \cellcolor{color_10_0!25} 100\% & \cellcolor{color_10_0!25} 100\% & \cellcolor{color_10_0!25} 100\% & \cellcolor{color_10_0!25} 100\%\\
Reverse & \cellcolor{color_10_0!25} 100\% & \cellcolor{color_10_0!25} 90\% & \cellcolor{color_10_0!25} 100\% & \cellcolor{color_10_0!25} 90\%\\
Addition & \cellcolor{color_10_4!25} 60\% & \cellcolor{color_10_0!25} 100\% & \cellcolor{color_10_6!25} 40\% & \cellcolor{color_10_0!25} 100\%\\
3-number Addition & \cellcolor{color_10_1!25} 80\% & \cellcolor{color_10_1!25} 80\% & \cellcolor{color_10_9!25} 10\% & \cellcolor{color_10_4!25} 60\%\\
Single Digit Multiplication & \cellcolor{color_10_0!25} 100\% & \cellcolor{color_10_0!25} 100\% & \cellcolor{color_10_10!25} 0\% & \cellcolor{color_10_10!25} 0\%\\
\hline 
\end{tabular}




==> experiments/table_contrastive_1000.tex <==
\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|lcc|}
\hline 
\multicolumn{1}{|l|}{\backslashbox{Task}{Penalty on $Q(s, \bullet)$}} & No decay & Decay 
\\\hline 
Coping & \cellcolor{color_10_0!25} 100\% 10/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
Reverse & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
Reverse & \cellcolor{color_10_0!25} 100\% 10/10 & \cellcolor{color_10_0!25} 90\% 9/10\\
Walk & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_8!25} 20\% 2/10\\
Walk (FF) & \cellcolor{color_10_4!25} 60\% 6/10 & \cellcolor{color_10_6!25} 40\% 4/10\\
walk3 & \cellcolor{color_10_9!25} 10\% 1/10 & \cellcolor{color_10_1!25} 80\% 8/10\\
walk3_ff & \cellcolor{color_10_0!25} 100\% 10/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
Addition & \cellcolor{color_10_6!25} 40\% 4/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
3-number Addition & \cellcolor{color_10_9!25} 10\% 1/10 & \cellcolor{color_10_4!25} 60\% 6/10\\
Single Digit Multiplication & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
\hline 


==> experiments/table_contrastive_10000.tex <==
\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|lcc|}
\hline 
\multicolumn{1}{|l|}{\backslashbox{Task}{Penalty on $Q(s, \bullet)$}} & No decay & Decay 
\\\hline 
Coping & \cellcolor{color_10_0!25} 100\% 10/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
Reverse & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
Reverse & \cellcolor{color_10_0!25} 100\% 10/10 & \cellcolor{color_10_0!25} 90\% 9/10\\
Walk & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_8!25} 20\% 2/10\\
Walk (FF) & \cellcolor{color_10_4!25} 60\% 6/10 & \cellcolor{color_10_6!25} 40\% 4/10\\
walk3 & \cellcolor{color_10_9!25} 10\% 1/10 & \cellcolor{color_10_1!25} 80\% 8/10\\
walk3_ff & \cellcolor{color_10_0!25} 100\% 10/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
Addition & \cellcolor{color_10_6!25} 40\% 4/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
3-number Addition & \cellcolor{color_10_9!25} 10\% 1/10 & \cellcolor{color_10_4!25} 60\% 6/10\\
Single Digit Multiplication & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
\hline 


==> experiments/table_contrastive_95.tex <==
\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|lcc|}
\hline 
\multicolumn{1}{|l|}{\backslashbox{Task}{Penalty on $Q(s, \bullet)$}} & No decay & Decay 
\\\hline 
Coping & \cellcolor{color_10_0!25} 100\% 10/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
Reverse & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
Reverse & \cellcolor{color_10_0!25} 100\% 10/10 & \cellcolor{color_10_0!25} 90\% 9/10\\
Walk & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_8!25} 20\% 2/10\\
Walk (FF) & \cellcolor{color_10_4!25} 60\% 6/10 & \cellcolor{color_10_6!25} 40\% 4/10\\
walk3 & \cellcolor{color_10_9!25} 10\% 1/10 & \cellcolor{color_10_0!25} 90\% 9/10\\
walk3_ff & \cellcolor{color_10_0!25} 100\% 10/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
Addition & \cellcolor{color_10_4!25} 60\% 6/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
3-number Addition & \cellcolor{color_10_1!25} 80\% 8/10 & \cellcolor{color_10_1!25} 80\% 8/10\\
Single Digit Multiplication & \cellcolor{color_10_0!25} 100\% 10/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
\hline 


==> experiments/table_curriculum.tex <==
\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|lcc|}
\hline 
\multicolumn{1}{|l|}{\backslashbox{Task}{Curriculum}} & \multicolumn{1}{|c|}{off} & \multicolumn{1}{|c|}{on}\\\hline 
3-number Addition & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_1!25} 80\% 8/10\\
\hline 


==> experiments/table_more_reward.tex <==
\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|lccc|}
\hline 
\multicolumn{1}{|l|}{\backslashbox{Task}{Reward Type}} & \multicolumn{1}{|c|}{0/1 reward} & \multicolumn{1}{|c|}{Discretized reward} & \multicolumn{1}{|c|}{Continuous reward}\\\hline 
Coping & \cellcolor{color_10_4!25} 0.6 & \cellcolor{color_10_4!25} 0.6 & \cellcolor{color_10_5!25} 0.8\\
Reverse & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0\\
Reverse & \cellcolor{color_10_2!25} 3.1 & \cellcolor{color_10_2!25} 3.1 & \cellcolor{color_10_10!25} 59.7\\
Walk & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0 & \cellcolor{color_10_1!25} 250.0\\
Walk (FF) & \cellcolor{color_10_7!25} 250.0 & \cellcolor{color_10_0!25} 14.5 & \cellcolor{color_10_7!25} 250.0\\
walk3 & \cellcolor{color_10_0!25} 7.5 & \cellcolor{color_10_9!25} 250.0 & \cellcolor{color_10_5!25} 162.8\\
walk3_ff & \cellcolor{color_10_2!25} 11.1 & \cellcolor{color_10_2!25} 9.5 & \cellcolor{color_10_10!25} 250.0\\
Addition & \cellcolor{color_10_2!25} 21.1 & \cellcolor{color_10_3!25} 21.6 & \cellcolor{color_10_9!25} 24.2\\
3-number Addition & \cellcolor{color_10_2!25} 81.9 & \cellcolor{color_10_2!25} 77.9 & \cellcolor{color_10_10!25} 131.9\\
Single Digit Multiplication & \cellcolor{color_10_1!25} 24.7 & \cellcolor{color_10_6!25} 26.5 & \cellcolor{color_10_6!25} 26.6\\
\hline 


==> experiments/table_q_classic.tex <==
\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|lcc|}
\hline 
\multicolumn{1}{|l|}{\backslashbox{Task}{Discount}} & \multicolumn{1}{|c|}{0.95} & \multicolumn{1}{|c|}{Dynamic}\\\hline 
Coping & \cellcolor{color_10_0!25} 90\% 9/10 & \cellcolor{color_10_0!25} 90\% 9/10\\
Reverse & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
Reverse & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
Walk & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
Walk (FF) & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
walk3 & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
walk3_ff & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
Addition & \cellcolor{color_10_1!25} 80\% 8/10 & \cellcolor{color_10_4!25} 60\% 6/10\\
3-number Addition & \cellcolor{color_10_6!25} 40\% 4/10 & \cellcolor{color_10_5!25} 50\% 5/10\\
Single Digit Multiplication & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
\hline 


==> experiments/table_q_pulled.tex <==
\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|lcc|}
\hline 
\multicolumn{1}{|l|}{\backslashbox{Task}{$Q$-learning Type}} & \multicolumn{1}{|c|}{$Q$-learning} & \multicolumn{1}{|c|}{Watkins's $Q(\lambda)$}\\\hline 
Coping & \cellcolor{color_10_0!25} 90\% 9/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
Reverse & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
Walk & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10\\
Walk (FF) & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_4!25} 60\% 6/10\\
Addition & \cellcolor{color_10_4!25} 60\% 6/10 & \cellcolor{color_10_4!25} 60\% 6/10\\
3-number Addition & \cellcolor{color_10_5!25} 50\% 5/10 & \cellcolor{color_10_1!25} 80\% 8/10\\
Single Digit Multiplication & \cellcolor{color_10_0!25} 100\% 10/10 & \cellcolor{color_10_0!25} 100\% 10/10\\
\hline 


==> experiments/table_simple.tex <==
\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|lcccc|}
\hline 
\multicolumn{1}{|l|}{\backslashbox{Task}{Learning}} Big Network & \multicolumn{3}{|c|}{Classical Q-learning} & \multirow{2}{*}{Our enhanced $Q$-learning} 
\\\cline{1-4} 
 \multicolumn{1}{|l|}{Discount} & \multicolumn{1}{|c}{0.95} & 0.99 & \multicolumn{1}{c|}{No Discount} & \\
\hline 
walk3 & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_10!25} 0\% 0/10 & \cellcolor{color_10_0!25} 90\% 9/10\\
\hline 


==> experiments/table_supervised.tex <==
\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|lcccc|}
\hline 
\multicolumn{1}{|l|}{\backslashbox{Task}{Unit}}FF & GRU & LSTM 
\\\hline 
Coping & 6.0 & 6.0 & 6.0\\
Reverse & 6.0 & 6.0 & 6.4\\
Walk & 12.8 & 18.8 & 29.6\\
Addition & Unsolvable & 18.8 & 14.4\\
3-number Addition & Unsolvable & 21.6 & 26.8\\
Single Digit Multiplication & Unsolvable & 102.0 & 41.2\\
\hline 


==> old/algorithms_as_an_finite_state_automata.tex <==
\section{Algorithms as an finite state automata}
Execution of an algorithm corresponds to transition in finite state automata. Model has to learn how to mimic automata
in order to solve algorithmical problem. States of model are self-contain, and should be mapped to the states of the algorithm 
corresponding automata. One of problems that we consider to reverse string. This corresponds to an automata Figure \ref{fig:reverse_automata}.
Transition between states should occur once model reaches end-of-sequence, then it should start going to the left. Expressive Controllers like
LSTM tend to learn an incorrect automata (Figure \ref{fig:wrong_automata}). They count how often they stayed in the state ``Go right'', and based
on it they estimate probability of transition to the next state. They combine this probabilities with occurence of the clue (i.e. end-of-sequence).
Correct solution should be based purely on clue.


\begin{figure}
  \begin{center}
    \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=2cm]
      \node[state,accepting] (A)      {{\tiny Go right}};
      \node[state]         (B) [right of=A]  {{\tiny Go left}};
      \path[->] (A)  edge [loop above] node {} (A)
                     edge              node {} (B)
                (B)  edge [loop above] node {} (B);
    \end{tikzpicture}
  \end{center}

  \caption{Automata describing correct solution to the {\textit reverse} problem. Model first has to go the right, and suppress prediction.
Then it has to go the left and predict what it sees at the given moment.}
  \label{fig:reverse_automata}
\end{figure}


\begin{figure}
  \begin{center}
    \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=2cm]
      \node[state,accepting] (A0)                {{\tiny Go right$_1$}};
      \node[state]           (A1) [below of=A0]  {{\tiny Go right$_2$}};
      \node[state]           (A2) [below of=A1]  {{\tiny Go right$_3$}};
      \node[state]           (A3) [below of=A2]  {{\tiny Go right$_4$}};
      \node[state]           (B)  [right of=A0]  {{\tiny Go left}};
      \path[->]  (A0) edge              node {} (B)
                      edge              node {} (A1)
                 (A1) edge              node {} (B)
                      edge              node {} (A2)
                 (A2) edge              node {} (B)
                      edge              node {} (A3)
                 (A3) edge              node {} (B)
                 (B)  edge [loop above] node {} (B);
    \end{tikzpicture}
  \end{center}
  \caption{This is an incorrect automata to solve {\textit reverse} problem. However, expressive models like LSTM tent 
  to learn such incorrect automata.}
  \label{fig:wrong_automata}
\end{figure}


\subsection{Double bias-variance trade off}

Generalization can be achieved by limiting capacity of model, 
or providing more training data. However, it's out of our interest to use
low capacity models for algorithmical tasks, as we would like to eventually scale them
to very hard problems. Our results indicate that providing more training data 
doesn't help to solve problem. 
Large models end up learning \textit{state-transition probabilities}.


\begin{figure}
  \begin{center}
    \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=1.5cm]
      \node[state, fill=green]         (S1)      {$S_1$};
      \node[state, fill=green]         (S2) [right of=S1] {$S_2$};
      \node[state, fill=green]         (S3) [right of=S2] {$S_3$};
      \node[state, fill=green]         (S4) [right of=S3] {$S_4$};
      \node[state, fill=green]         (S5) [right of=S4] {$S_5$};
      \node[state, fill=green, accepting]         (S6) [right of=S5] {$S_6$};
      \path[->] (S1)  edge node {} (S2)
                (S2)  edge node {} (S3)
                (S3)  edge node {} (S4)
                (S4)  edge node {} (S5)
                (S5)  edge node {} (S6);

    \end{tikzpicture}
  \end{center}
  \caption{Evolution of state for RNN. Every state depends on all previous states. There is a mismatch between training, and
  test distribution of RNNs states. This is the cause of lack of generalization.}
  \label{fig:rnn}
\end{figure}


Typical algorithm solving model uses RNN as it's Controller. 
RNN consumes data, and state from the past time-step and derives new
time step (Figure \ref{fig:rnn}).
This means that during testing states are
iterated many more times in compare to training. 
Main reason why models fail to generalize to inductive patterns is mismatch 
between training and testing procedure.


\begin{figure}
  \begin{center}
    \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=1.5cm]
      \node[state]         (S1)      {$S_1$};
      \node[state]         (S2) [right of=S1] {$S_2$};
      \node[state]         (S3) [right of=S2] {$S_3$};
      \node[state]         (S4) [right of=S3] {$S_4$};
      \node[state]         (S5) [right of=S4] {$S_5$};
      \node[state, fill=green, accepting]         (S6) [right of=S5] {$S_6$};
    \end{tikzpicture}
  \end{center}
  \caption{Evolution of state for feed-forward network. Every state is completely independent. 
  There is no information passed between time-steps. This model can generalize to an arbitrary length of sequences, 
  because there is match between training and test distribution for it's states. It can learn simple patterns like given
  digit $n \in [0, \dots 8]$ predict $n+1$. However, it cannot learn any patterns that are dependent on several time-steps.}
  \label{fig:ff}
\end{figure}



There are many other models that can operate on sequences that would have a match
between training, and test distribution of states regardless of sequence length. 
The simplest example is the feed-forward network, which consumes current input
regardless of past (Figure \ref{fig:ff}). Such model is quite weak, as it can solve
problems that doesn't have any time dependency. However, for problems that it can
solve, it generalizes to an arbitrary length, as the training states look the same 
as test states.


\begin{figure}
  \begin{center}
    \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=1.5cm]
      \node[state]         (S1)      {$S_1$};
      \node[state]         (S2) [right of=S1] {$S_2$};
      \node[state]         (S3) [right of=S2] {$S_3$};
      \node[state, fill=green]         (S4) [right of=S3] {$S_4$};
      \node[state, fill=green]         (S5) [right of=S4] {$S_5$};
      \node[state, fill=green, accepting]         (S6) [right of=S5] {$S_6$};

      \path[->] (S4)  edge node {} (S5)
                (S5)  edge node {} (S6);

    \end{tikzpicture}
  \end{center}
    \caption{Evolution of state for feed-forward network over short past. Every state depends only on few states from the past.
    We assume that it depends on fewer states than length of training examples.
    This model can generalize to an arbitrary length of sequences, because there is match between training and test distribution for it's states.
    It can learn patterns like repeat last few characters. However, it cannot learn long-term dependencies, like to remember to close a bracket after many
    time-steps.}
  \label{fig:many_ff}
\end{figure}

Another trivial model that has inductive generalization property is feed-forward network
over few last time-steps (Figure \ref{fig:many_ff}). We assume that number of time-steps that it consumes is smaller than
length of training sequence. This model is slightly more powerful than feed-forward network
over last time step. For instance, it can learn to repeat short sequences, which wouldn't 
be feasible for feed-forward network over last time-step. However, it cannot model tasks that
require long distance dependency, like to remember to close a bracket. 


\begin{figure}
  \begin{center}
    \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=1.5cm]
      \node[state]         (S1)      {$S_1$};
      \node[state]         (S2) [right of=S1] {$S_2$};
      \node[state, fill=green]         (S3) [right of=S2] {$S_3$};
      \node[state, fill=green]         (S4) [right of=S3] {$S_4$};
      \node[state]         (S5) [right of=S4] {$S_5$};
      \node[state, fill=green, accepting]         (S6) [right of=S5] {$S_6$};
    \end{tikzpicture}
  \end{center}
  \caption{Final state is dependent on few past inputs. Past inputs are chosen using sparse attention.
  Such state would ``look'' the same regardless of input sequence length. This gives induction generalization property. This model
  is strictly more powerful than feed-forward network over last few states, however is weaker than RNN. Nonetheless it has
  natural tendency to generalize to inductive patterns.}
  \label{fig:sam}
\end{figure}



We propose new model \textit{Sparse Attention Model} (SAM) that has inductive generalization properties (Figure \ref{fig:sam}).  
SAM does soft-attention over past time-steps, and it picks fixed number of most responsive locations.
This way it can model long term dependencies, and test data distribution of states matches train data distribution of states. 
Few tricks allow to further extend expressive power. One is to provide few tokens to do relative addressing (following \cite{sukhbaatar2015weakly}).
This allows to access state $T - 1$, or $T - 2$. Beyond some relative time all states have the same token.
Second trick to extend expressive power is to have multiple hops. It means that controller can look into past locations multiple times. 




==> old/attention_as_state_carrier.tex <==
\section{Attention as state carrier}

\subsection{Sparse attention}

\subsection{Time tokens}

\subsection{Hops}




==> old/colors.tex <==
\definecolor{color3}{rgb}{0.000, 0.000, 1.000}
\definecolor{color4}{rgb}{0.000, 0.059, 0.941}
\definecolor{color5}{rgb}{0.000, 0.118, 0.882}
\definecolor{color6}{rgb}{0.000, 0.173, 0.827}
\definecolor{color7}{rgb}{0.000, 0.231, 0.769}
\definecolor{color8}{rgb}{0.000, 0.286, 0.714}
\definecolor{color9}{rgb}{0.000, 0.345, 0.655}
\definecolor{color10}{rgb}{0.000, 0.400, 0.600}
\definecolor{color11}{rgb}{0.000, 0.459, 0.541}
\definecolor{color12}{rgb}{0.000, 0.518, 0.482}
\definecolor{color13}{rgb}{0.000, 0.573, 0.427}
\definecolor{color14}{rgb}{0.000, 0.631, 0.369}
\definecolor{color15}{rgb}{0.000, 0.686, 0.314}
\definecolor{color16}{rgb}{0.000, 0.745, 0.255}
\definecolor{color17}{rgb}{0.000, 0.804, 0.196}
\definecolor{color18}{rgb}{0.000, 0.859, 0.141}
\definecolor{color19}{rgb}{0.000, 0.918, 0.082}
\definecolor{color20}{rgb}{0.000, 0.973, 0.027}
\definecolor{color21}{rgb}{0.027, 0.973, 0.000}
\definecolor{color22}{rgb}{0.082, 0.918, 0.000}
\definecolor{color23}{rgb}{0.141, 0.859, 0.000}
\definecolor{color24}{rgb}{0.196, 0.804, 0.000}
\definecolor{color25}{rgb}{0.255, 0.745, 0.000}
\definecolor{color26}{rgb}{0.314, 0.686, 0.000}
\definecolor{color27}{rgb}{0.369, 0.631, 0.000}
\definecolor{color28}{rgb}{0.427, 0.573, 0.000}
\definecolor{color29}{rgb}{0.482, 0.518, 0.000}
\definecolor{color30}{rgb}{0.541, 0.459, 0.000}
\definecolor{color31}{rgb}{0.600, 0.400, 0.000}
\definecolor{color32}{rgb}{0.655, 0.345, 0.000}
\definecolor{color33}{rgb}{0.714, 0.286, 0.000}
\definecolor{color34}{rgb}{0.769, 0.231, 0.000}
\definecolor{color35}{rgb}{0.827, 0.173, 0.000}
\definecolor{color36}{rgb}{0.882, 0.118, 0.000}
\definecolor{color37}{rgb}{0.941, 0.059, 0.000}
\definecolor{color38}{rgb}{1.000, 0.000, 0.000}


==> old/induction_friendly_q_learning.tex <==
\section{Induction friendly Q-learning}


==> old/introduction.tex <==
\section{Introduction}

Learning patterns that extend far beyond training data distribution 
requires understanding which properties of training data 
will stick beyond training distribution. 
For instance, given that training data consist of sequences of length up to 
$10$, model can learn that it is likely to terminate prediction after reading $10$
words. We found that indeed expressive models tend to learn such
\textit{state transition probabilities}. This property is undesired 
if we expect model to learn non-deterministic, algorithmical pattern.


Algorithmal patterns like how to add decimal numbers are equivalent of learning
deterministic finite state automata. For instance, adding two numbers has several states:
(1) read digit of the upper number, (2) read digit of the lower number
(3) add digits and previously stored carry, (4) produce output
(5) store carry, (6) move to the digit to the left, and (6) repeat until end of sequence.
Training data might consist of numbers up to length $5$. Expressive model can learn on top of this rules that
after reading $5$-th digit it is likely to terminate. Learnt pattern decomposes as a combination of:
(1) transition probability, and (2) occurrence of the clue.


Aforementioned, property has far-reached consequences. Large, expressive models might have a trouble 
learning algorithmical patterns, because they end up learning \textit{too much}. They learn transition
probability between states, which is present in training data. To circumvent it, previous models had to limit
their expressive power. For instance,
Neural Turing Machine \cite{graves2014neural} had to be \textit{crippled} to make it work. It got
\textit{crippled} by removing recurrent connections, and changing LSTM to an another gating function (likely less powerful).
Stack RNN \cite{joulin2015inferring} researchers used tiny RNNs in their experiment ($30$ units). 
The success of previous models is due to tiny size, and making them less powerful. However, learning complex
algorithmical patterns is likely to require huge, unconstrained models. 
It's important to note that stated property of big models is not just in over-fitting. Big models regardless of 
amount of training data end up learning state-transition probabilities. Big models have an inductive bias to learn
undesired patterns.


Our contribution is in 
\begin{itemize}
  \item identifying problem of learning state-transition probabilities 
  \item proposing class of large models that can learn inductive pattens regardless of model size.
  \item induction friendly Q-learning
\end{itemize}
Lastly, we would like to direct the reader to the video
accompanying this paper (\url{http:\\\\youtube.com}). The code for this work can be found at \url{https://github.com/wojzaremba/mem}.





==> old/model.tex <==
\section{Model}

\begin{figure}
  \begin{center}
    \begin{picture}(200, 130)
      \put(74, 60){\framebox(52, 15){}}
      \put(86, 65){{\scriptsize \textbf{Controller}}}
      \put(74, 50){\framebox(52, 10){}}
      \put(77, 53){{\scriptsize Controller Input}}
      \put(74, 75){\framebox(52, 10){}}
      \put(75, 78){{\scriptsize Controller Output}}

      \put(50, 15){\vector(1, 1){34}}
      \put(19, 0){\framebox(52, 15){}}
      \put(24, 5){{\scriptsize Input Interface}}


      \put(100, 15){\vector(0, 1){34}}
      \put(74, 0){\framebox(52, 15){}}
      \put(77, 5){{\scriptsize Output Interface}}


      \put(150, 15){\vector(-1, 1){34}}
      \put(129, 0){\framebox(52, 15){}}
      \put(130, 5){{\scriptsize Memory Interface}}

      \put(90, 85){\vector(-1, 1){34}}
      \put(19, 119){\framebox(52, 15){}}
      \put(24, 124){{\scriptsize Input Interface}}


      \put(100, 85){\vector(0, 1){34}}
      \put(74, 119){\framebox(52, 15){}}
      \put(77, 124){{\scriptsize Output Interface}}


      \put(115, 85){\vector(1, 1){34}}
      \put(129, 119){\framebox(52, 15){}}
      \put(130, 124){{\scriptsize Memory Interface}}


      \put(40, 68){\vector(1, 0){33}}
      \put(127, 68){\vector(1, 0){33}}
      \put(11, 66){{\scriptsize Past State}}
      \put(164, 66){{\scriptsize Future State}}

    \end{picture}
  \end{center}
  \caption{Figure presents generic model to solve algorithmical problems. It consists of (1) Controller, and (2) Interfaces. A typical Interface is
  a memory, or stack. Interfaces expose API, and Controller uses API to access content. Controller passes state between time steps.
  Entire model is usually trained with SGD.}
  \label{fig:interfaces}
\end{figure}



Models solving algorithmical problems
can be abstracted as a combination of \textbf{Controller}, and \textbf{Interfaces} (Figure \ref{fig:interfaces}).
Controller consumes current time step information
from Interfaces, and provides actions over them. Actions are either continuous, or
discrete. Where discrete actions requires reinforcement learning, or target propagation.
Moreover, we consider input as an Input Interface that provides
input data symbols (usually consecutive symbols).
Output is also an Interface, that usually becomes active after entire input consumption.
Quite often Output Interface provides correct predictions for the last time step as an input (``teacher force'').


For instance, Memory Network has feed forward network as a controller, and 
two interfaces such as (1) input interface, which is accessible with soft-attention,
and (2) output interface over which MN provides predictions.

Neural Turing Machine has a LSTM as a Controller, and 
three interfaces such as (1) input interface, which consumes consecutive input symbols,
(2) output interface over which NTM provides predictions, and (3) grid of values of memory.



Prior work was concerned with providing better Interfaces (Stack vs Grid vs Queue), or better
learning algorithm (SGD, search, reinforcement learning). However, we show the bottleneck in
training is in the Controller. Over-expressive controller like RNN or LSTM make training difficult
due to lack of inductive generalization. 


\subsection{Interfaces}
We consider various interfaces in this work. Available interfaces are dependent
on task that we are solving.


\subsubsection{Input tape}
Data is provided as sequence. Model sees a single character at the time. 
Controller decides to move either (1) move to the left, (2) stay, or (3) move to the right. 
For instance, reverting sequence requires to get to the end of sequence by going to the right.
Then model should keep on going to the left. This interface is not mandatory. When it's off
data is provided sequentially from left to right.

\subsubsection{Input grid}
Data is provided on two-dimensional grid. Model sees a single character at the time.
Controller decides to move either (1) to the left, (2) stay, (3) to the right, (4) up, (5) down, or over diagonals 
(in total $9$ possible actions). 
Solving addition is much simpler with such interface in compare to tape. 
(assuming that numbers are provided one under another).

\subsubsection{Output interface}
Output interface allows to decide when to make a prediction. At every time step model can decide either to make
a prediction, or not. If Output interface is off then model has to make a prediction at every time step. 
This interface unleashes unbounded computational time for this model. Together with Memory interface makes model
Turing complete.

\subsubsection{Memory Tape}
Memory allows to save, and load symbols from the input. Controller can either save or not, and decide (1) to go the left,
(2) stay, (3) go to the right. 



==> old/related_work.tex <==
\section{Related work}
There has been many models designed to solve algorithmical patterns like 
Neural Turing Machine \cite{graves2014neural},
Stack RNN \cite{joulin2015inferring},
LSTM \cite{zaremba2014learning}, 
Reinforcement Learning Neural Turing Machine \cite{zaremba2015reinforcement},
Weakly supervised Memory Networks \cite{sukhbaatar2015weakly},
, and Neural DeQue \cite{grefenstette2015learning}. 
They consider solving simple algorithmical tasks like addition, coping, reverting sequences, 
and sequence transduction problems. The main interest is in
proving more powerful interfaces, and proposing better learning algorithm.
All this models apart from \cite{sukhbaatar2015weakly} are based on RNN as the core
computational unit. We show that one of critical problems is in choosing RNN as the
core computational unit. Controller considerations were out of interest for previous work. 



Learning algorithms is closely related with learning automata. 
There has been extensive work in this topic \cite{narendra2012learning, najim2014learning}.
However, previous work either (1) searches for automata by exhaustively enumerating them, 
(2) does hill climbing in the space of automata, or (3) fixes automata and learns transition
weights. We believe, that explicit enumeration and search in this space might be difficult, as 
the space is quite discontinuous. We prefer to parameterize an algorithm using neural network, and
implicitly search space of automata. 





==> old2/model.tex <==
\section{Model}
\label{sec:model}
A complicated tasks require multi-step interaction with an external environment, such as 
a computer game (\cite{mnih2013playing}), a stock exchange, an advertisement system, or the physical world (robotics).  
A model can read the partial state from the environment, and influence the environment by applying 
actions. We formalize this concept under name Interface--Controller interaction.



The external environment is available through Interfaces that expose
API. For instance, human accesses world by senses such as eyes Interface and 
touch Interface, and others. Touch Interface provides methods to contract muscles, and
to return current muscle contraction, pain level, temperature and few others.
In our examples, we define simplistic Interfaces that allow to control access to the input data, and to  
spin computation for multiple time-steps.


The part of the model that communicates with Interfaces is called the Controller. The Controller is the only
part of the system which learns. The Controller can have prior knowledge about behaviour of Interfaces
or not. In all our examples, we start with a clean slate and provide no prior knowledge about any of Interfaces. 
The Controller learns sequence of actions over Interfaces that allow to 
solve a task. Figure \ref{fig:interfaces} presents full Interfaces--Controller abstraction together
with an example.





The prior work has considered models with various Interfaces. However, this concept 
was never considered as separate, fundamental entity. 
For instance, Memory Network (\cite{weston2014memory}) has a feed forward network as a Controller, and 
two Interfaces such as (1) input Interface, which is accessible with soft-attention,
and (2) output Interface.
An another example is Neural Turing Machine (\cite{graves2014neural}). This model has a modified LSTM as a Controller, and three 
Interfaces such as (1) input Interface,
(2) output Interface, and (3) memory Interface.



Further subsections describe Interfaces used in this work.
We consider Interfaces such as:
Input Tape Interface (Subsection \ref{subsubsec:input_tape}), 
Input Grid Interface (Subsection \ref{subsubsec:input_grid}) and 
Output Tape Interface (Subsection \ref{subsubsec:output_tape}). 




\begin{figure}
  \begin{center}
    \scalebox{0.65}{
      \begin{picture}(200, 130)
        \put(74, 60){\framebox(52, 15){}}
        \put(86, 65){{\scriptsize \textbf{Controller}}}
        \put(74, 50){\framebox(52, 10){}}
        \put(77, 53){{\scriptsize Controller Input}}
        \put(74, 75){\framebox(52, 10){}}
        \put(75, 78){{\scriptsize Controller Output}}

        \put(50, 15){\vector(1, 1){34}}
        \put(19, 0){\framebox(52, 15){}}
        \put(24, 5){{\scriptsize Input Interface}}


        \put(100, 15){\vector(0, 1){34}}
        \put(74, 0){\framebox(52, 15){}}
        \put(77, 5){{\scriptsize Output Interface}}


        \put(150, 15){\vector(-1, 1){34}}
        \put(129, 0){\framebox(52, 15){}}
        \put(130, 5){{\scriptsize Memory Interface}}

        \put(90, 85){\vector(-1, 1){34}}
        \put(19, 119){\framebox(52, 15){}}
        \put(24, 124){{\scriptsize Input Interface}}


        \put(100, 85){\vector(0, 1){34}}
        \put(74, 119){\framebox(52, 15){}}
        \put(77, 124){{\scriptsize Output Interface}}


        \put(115, 85){\vector(1, 1){34}}
        \put(129, 119){\framebox(52, 15){}}
        \put(130, 124){{\scriptsize Memory Interface}}


        \put(40, 68){\vector(1, 0){33}}
        \put(127, 68){\vector(1, 0){33}}
        \put(11, 66){{\scriptsize Past State}}
        \put(164, 66){{\scriptsize Future State}}

      \end{picture}
    }
    \includegraphics[width=0.6\linewidth]{stills/full.png}
  \end{center}
  \caption{This figure presents an overview of the model based on Interfaces--Controller abstraction.
  \textbf{(Left)} shows an abstract model, and \textbf{Right} shows an instantiation
  of the model on an addition task. 
  The entire system evolves over the time, and arrows indicate information flow. 
  The left image presents model at a given time-step, 
  while right image presents three time-steps of the model evolution.
  The bottom, middle, and the top of both figures corresponds to each other.
  \textbf{(Bottom)} reads methods exposed by Interfaces, \textbf{(Middle)} 
  the Controller, and \textbf{(Top)} write methods exposed by Interfaces.
  The common choice for the Controller is a RNN (for instance, GRU as on the right image).}
  \label{fig:interfaces}
\end{figure}





\subsection{Input tape}
\label{subsubsec:input_tape}
The Input Tape provides access to the input data symbols stored on an ``infinite'' tape.
This Interface allows to read a single character from the current head location
by calling \textit{read()} method. The head can be moved by calling
\textit{move} method of the Input Tape. The \textit{move} method takes one of the following 
arguments: \textit{left} or \textit{right} (Figure \ref{fig:input}). 
This interface is similar to an abstract Tape envisioned by Alan Turing (\cite{turing1936computable}).
Our version is impoverished, and doesn't allow to change content of the tape.


Solving task like reverting sequence requires several steps of interaction with this Interface.
First, Controller has to move the head to the end of sequence by
calling \textit{move(right)} multiple times. On this stage, seen symbols should be discarded.
Then, after reaching the end of the sequence, the Controller has to request \textit{move(left)}
multiple times. On the way left, the Controller has to \textit{read()} characters from the Input Tape, and write 
them to the Output Tape.



\subsection{Input grid}
\label{subsubsec:input_grid}
The Input Grid provides access to the input data symbols stored on an ``infinite'' grid.
This Interface allows to read a single character from the current head location.
The head can be moved by calling \textit{move}
method with argument: \textit{up}, \textit{left}, \textit{down} or \textit{right} 
(Figure \ref{fig:input}). 
This Interface is similar to a piece of paper for human. 


The task of addition of multi-digit numbers is much simpler with such interface in compare to a tape
(assuming that numbers are provided one under another).
This task has smaller computational complexity when Input Grid is available in compare to the
Input Tape. 



\begin{figure}
  \centering
  \fbox{
    \begin{minipage}[t]{0.48\linewidth}
      \begin{center}
        \vspace{7mm}
        \includegraphics[width=0.23\linewidth]{stills/tape/tape_1.png}
        \includegraphics[width=0.23\linewidth]{stills/tape/tape_2.png}
        \includegraphics[width=0.23\linewidth]{stills/tape/tape_3.png}
        \includegraphics[width=0.23\linewidth]{stills/tape/tape_4.png}
        \vspace{4.25mm}
        \\
        {\small Input Tape\\}
        \vspace{1mm}
      \end{center}
    \end{minipage}
  }
  \fbox{
    \begin{minipage}[t]{0.48\linewidth}
      \begin{center}
        \vspace{1mm}
        \includegraphics[width=0.23\linewidth]{stills/grid/grid_1.png}
        \includegraphics[width=0.23\linewidth]{stills/grid/grid_2.png}
        \includegraphics[width=0.23\linewidth]{stills/grid/grid_3.png}
        \includegraphics[width=0.23\linewidth]{stills/grid/grid_4.png}
        \\
        {\small Input Grid\\}
        \vspace{1mm}
      \end{center}
    \end{minipage}
  }
  \caption{Input Interfaces provide access to the training data. They also specify
\textit{move} method to navigate over them. We consider \textbf {(Left)} the Input Tape, and 
\textbf{(Right)} the Input Grid. Both of this Interfaces have a reading head that delivers a single character
at the time-step. We marked reading head with a yellow box. Stills present four time-steps for each of Interfaces.
\textit{move} method for the Input Tape takes arguments \textit{left}, or \textit{right}.
Where for the Input Grid it takes arguments: \textit{up}, \textit{left}, \textit{down} or \textit{right}.}
  \label{fig:input}
\end{figure}



\subsection{Output tape}
\label{subsubsec:output_tape}
The Output Interfaces allows to write a structured answer. 
For instance, if the answer would have to be a tree, then the Output Interface would provide
actions to navigate such tree, and write over the nodes. 
Moreover, the Output Interface provides the learning signal
by comparing written answers to the target symbols (when we assume supervised setting). 
This learning signal can be differentiable (for instance, cross-entropy).


The most common case of the Output Interface is the Sequential Output Interface.
The model has to write to this Interface at the every time step (as in case of language modelling). 
The another common option is Delayed Output Interface. This Interface expects sequence of outputs after consuming entire input sequence. 
This is common choice in the machine translation domain (\cite{sutskever2014sequence}).

 
We consider the Output Tape Interface, which is an extension of Sequential Output Interface,
and Delayed Output Interface. We call it the Output Tape Interface.
This Interface has two methods. 
First, the \textit{predict} method with arguments \textit{now} or \textit{later}.
The reward is given only when the Controller calls \textit{predict(now)}. 
We require our model to call \textit{predict(now)} at
least once per sample. This constraint is necessary to get any learning signal.
Second, the \textit{write} method with arguments of size of the vocabulary.
The Output tape advances only forward. It's forbidden to modify already emitted symbols.




Th Output Tape Interface enables unbounded computational time, as predictions can be postponed.
Some problems like sorting by comparison requires minimum $\mathcal{O}(n \log n)$ operations\footnote{``Bucket 
sort'' sorts numbers in $\mathcal{O}(n)$ however range of numbers has to be small, and fixed.} (\cite{cormen2009introduction}).
However in practise, none of our tasks requires more than $\mathcal{O}(n)$ computational steps. 
We were not able to solve any task with higher computational complexity.





==> old2/q_learning.tex <==
\section{$Q$-learning}
\label{sec:q_learning}
The previous Sections describes the upper bound on the performance of our system. 
We considered the setting where all actions are provided, and the model doesn't have to guess them.
Following Sections concern training where actions are not given. The model
has to learn solely from pairs of sequences over the Input Interface, and desired 
sequences over the Output Interface. We rely on modified $Q$-learning. Following Sections
describe $Q$-learning, and the enhancements that we consider.




$Q$-learning is the classical reinforcement learning algorithm. It involves learning $Q$ function
that estimates the sum of the future rewards. $Q$ is indexed by the current state $s$ and the undertaken action $a$. 
The update of $Q(s, a)$ is described by the equation:
\begin{align*}
  Q_{n + 1}(s, a) = Q_n(s, a) - \alpha \big[Q_n(s, a) - \big(R(s') + \max_{a}Q_n(s', a)\big)\big]
\end{align*}
Taking the action $a$ in state $s$ cause transition to the state $s'$.
$R(s')$ is a reward experienced in the state $s'$. 
The another commonly considered quantity is $V(s) = \max_a Q(s, a)$. 
$V$ is called the value function, and $V(s)$ is the expected sum of
future rewards starting from the state $s$. Moreover, $Q^*$ and $V^*$ 
are function values for the optimal policy.


Our agent experiences a reward of $1$ every time it makes a correct prediction. 
The incorrect prediction results in a zero reward.
Our tasks require precise predictions, and even a single mistake ruins the execution. 
We terminate an episode when incorrect prediction is made.
Moreover, we use slightly different strategy to learn targets.
We use the cross-entropy loss to compare predictions to targets, and we 
backpropagate this objective. This is prevalent loss function in the supervised learning.
Thus RL is really used here because we have discrete Interfaces.


The amount of positive reward depends on the progress of the learning. At the very beginning,
the model is unlikely to receive many positive rewards, because most of predictions
are incorrect. The model would receive a very small positive reward even for 
the right sequence of actions.
The reward is dependent on the correct predictions of the target, and this improves 
over the time. Such setting defines a \textit{non-stationary} environment.
However, every RL algorithm assumes a \textit{stationary} environment. 
We propose to use Watkins's $Q(\lambda)$ \cite{sutton1998reinforcement}
instead of the classical $Q$-learning to mollify issue with a \textit{non-stationary} environment. 
Watkins's $Q(\lambda)$ relies much more
on the contemporary rewards over the estimated $Q$ values (Subsection \ref{subsec:pulled}).


We achieved boost in performance by reparametrizing $Q$ to be time invariant.
(Subsection \ref{subsec:reparametrization}).
Moreover, we exercise an ad hoc solution to achieve 
better generalization by having contrastive term on $Q(s, \bullet)$
(Subsection \ref{subsec:contrastive}).



\subsection{Time invariant $Q$}
\label{subsec:reparametrization}
The classical $Q$-function estimates the sum of the future rewards (or the discounted sum). 
This quantity is dependent on the remaining episode length. We reparametrize $Q$ to be
independent of the remaining episode length.
This is achieved by rescaling $Q$ according to the number of predictions that are
left until the end of episode. This quantity in known during training.


We know the total number of targets left until the end of the episode. This
quantity is equal to the overall number of target symbols minus the number of emitted symbols. 
Moreover, if none of the target predictions is guessed by luck, then this quantity is equal to $V^*(s)$ 
(every correct prediction is worth reward of $1$). We reparametrize $Q$ to:
\begin{align*}
  \hat{Q}(s, a) &:= \frac{Q(s, a)}{V^*(s)} \text{,  } \hat{Q}(s, a) \in [0, 1] \\
  \hat{Q}(s, a) &= \frac{R(s')}{V(s)} + \max_{a}\frac{V^*(s')}{V^*(s)} \hat{Q}(s', a) \\
  \hat{Q}_{n + 1}(s, a) &= \hat{Q}_{n}(s, a) - \alpha\big[\hat{Q}_{n}(s, a) - \big(\frac{R(s')}{V(s)} + \max_{a}\frac{V^*(s')}{V^*(s)} \hat{Q}_n(s', a)\big)\big]
\end{align*}
% WZ: Hard to plot anything.

$\frac{V^*(s')}{V^*(s)}$ is equal $1$ if there is no prediction between states $s$, and $s'$. 
$Q_n$ is copied to $Q_{n+1}$ whenever there is no prediction. 
The discount values $\frac{V^*(s')}{V^*(s)}$ are descending as episode progresses.
The model becomes greedier toward the end of episode. 
The discount at the end of episode becomes as small as $\frac{1}{2}$.
There is no reason not be greedy as the episode is almost over.


\subsection{Watkins's $Q(\lambda)$}
\label{subsec:pulled}
The rewards are self-generated by our model, and rewards frequency 
change as the model predictions improve.  
This behaviour is present regardless if chosen sequence of actions is right or not.
An execution of the correct sequence of actions at the beginning of training gives different amount of reward
in compare to the same sequence of actions for the trained model. This defines 
a \textit{non-stationary} environment. 
We propose to use 
Watkins's $Q(\lambda)$ to mollify issue of the \textit{non-stationary} environment.


\begin{figure}[h]
  \centering
  \includegraphics[width=0.35\linewidth]{img/watkins.png}
  \caption{The backup diagram for Watkins's $Q(\lambda)$. 
           Figure derived from the figure from \cite{sutton1998reinforcement}.}
  \label{fig:watkins}
\end{figure}


All RL algorithms assume a \textit{stationary} environment. However, 
our setting breaks this assumption. We have found that 
Watkins's $Q(\lambda)$ outperforms classical $Q$-learning 
in such situation. 
Watkins's $Q(\lambda)$ regresses on the larger number of contemporary rewards than the 
classical $Q$-learning. This promotes adjusting to the current environment
over sticking to the outdated $Q$ values.


Watkins's $Q(\lambda)$ uses multiple-step backup until non-greedy action is taken (Figure \ref{fig:watkins}).
Let's assume that greedy action has been taken in $n$-th step.
Moreover, we set $\lambda = 1$ in all our experiments, so we describe Watkins's $Q(\lambda)$ only for such $\lambda$:
\begin{align*}
  i &= 1, 2, \dots, n \\ 
  a_{t + i} &= \argmax_a Q(s_{t + i}, a) \\ 
  s_{t + i} &\xrightarrow{a_{t + i}} s_{t + i + 1}\\
  s_{t + n} &\nrightarrow{a_{t + n}} s_{t + n + 1}\\
  Q^*(s_t, a_t) &= \sum_{i=1}^T R(s_{t + i}) + \max_{a}Q^*(s_{t + n + 1}, a) \\ 
  Q_{n + 1}(s_t, a_t) &= Q_n(s_t, a_t) - \alpha\big[Q_n(s_t, a_t) - \big(\sum_{i=1}^n R(s_{t + i}) + \max_{a}Q_n(s_{t + n + 1}, a)\big) \big]
\end{align*}


Watkins's $Q(\lambda)$ ``unrolls'' rewards until non-greedy action is taken.
However, $\epsilon$-greedy policies chooses the greedy actions most of the time. 
They allows to unroll for approximately $\sim \frac{1}{\epsilon}$ steps.
Usually $\epsilon = 5\%$, which means that we can accumulate rewards for approximately $20$
steps before taking $\max$ over $Q$.


XXXXXXXXXXX continue here.

\subsection{Penalty on $Q(s, \bullet)$}
\label{subsec:contrastive}
Lack of out of training generalization might be caused by choosing incorrect action.
Actions during test are chosen from $\argmax_a Q(s, a)$. However, $Q(s, \bullet)$ is 
not normalized, and incorrect actions might not have enough margin from the correct one.
Penalty on $Q(s, \bullet)$ ensures that there is a slack between
correct, and incorrect actions. This greatly enhances generalization.



We assume that there is a single sequence of actions 
that leads to the solution. Optimal $Q$ after reparametrization (Subsection \ref{subsec:reparametrization})
should assign $1$ to the correct action, and $0$ to the incorrect one.
However, incorrect actions are visited less frequently than the correct one. 
Given that we use $\epsilon$-greedy policy with $\epsilon=5\%$, we visit incorrect states
only $5\%$ of time. 


We propose to ``push down'' incorrect actions by introducing a penalty on
$\lambda||\sum_a Q(s, a) - 1||^2$. This introduces margin between correct and incorrect actions,
which greatly enhances generalization.
We start training with $\lambda=0$, and we make it non-zero when accuracy on short samples is good enough.
Introducing it too early in training harms learning.








==> old2/related_work.tex <==
\section{Related work}
\label{sec:related}
% Vision
\cite{turing1936computable} classified computational models, and proved that
the most powerful one is the Turing machine. However, the contemporary computers
are implementation-wise far from the proposed read-write tape. Turing
proposed the framework to operate in. Over the time, practitioners
proposed better Interfaces to access memory than tape (i.e. RAM).
They introduced advances that doesn't change computational complexity of computer, 
but constant factor efficiency (i.e. multiple levels of cache, branch prediction etc.).



Similarly, we think, that many cutting edge, present--day models can be seen by 
Interface--Controller abstraction (Section \ref{sec:model}).


% Other people models (verify interfaces).
\textbf{Neural Turing Machine} (NTM) (\cite{graves2014neural}) has a modified LSTM as the Controller, and three 
Interfaces such as: Sequential Input, Delayed Output, and Differentiable Memory.

\vspace{-2mm}
\textbf{Weakly supervised Memory Network} (\cite{sukhbaatar2015weakly}) has a feed forward 
network as the Controller, and 
two Interfaces such as Soft-attention Input,
and Delayed Output.

\vspace{-2mm}
\textbf{Stack RNN} (\cite{joulin2015inferring}) has a RNN as the Controller, and 
three Interfaces such as Sequential Input, Memory Stack and Sequential Output.

\vspace{-2mm}
\textbf{Reinforcement Learning Neural Turing Machine} (RLNTM) (\cite{zaremba2015reinforcement}) has a LSTM as the Controller, and 
three Interfaces such as Sequential Input, the Memory Tape and the Output Tape.

\vspace{-2mm}
\textbf{Neural DeQue} (\cite{grefenstette2015learning}) has a LSTM as the Controller, and 
three Interfaces such as Sequential Input, the Memory Queue and the Sequential Output.

\vspace{-2mm}
\textbf{Our model} fits into 
the Interfaces--Controller abstraction. It has GRU as the Controller (or feed forward network),
and two Interfaces such as Input Tape / Grid, and Output Tape. 




Most of the prior work considered continuous Interfaces,
while we consider discrete Interfaces (similarly as \cite{zaremba2015reinforcement}).
Discrete Interfaces are empirically more challenging to train.
However, many external Interfaces are set to be discrete, and humans can use them anyway. 
For instance, Google search engine provides discrete actions. Human doesn't need to backpropagate
through search results to know how to use Google. 




% Q-learning.
We train the Controller to approximate $Q$-function (similarly to \cite{mnih2013playing}). 
However, we have introduced several modifications on top of classical $Q$-learning.
First, we use Watkins's $Q(\lambda)$ \cite{sutton1998reinforcement}. This helps to
overcome \textit{non-stationary} environment. We are unaware of any prior work that
uses Watkins's $Q(\lambda)$ for this purpose. Moreover, Watkins's $Q(\lambda)$ can be seen 
a method to form ``macro'' actions \cite{mcgovern1998macro, mcgovern1997roles, mcgovern2001automatic}.
Second, we reparametrized $Q$ function, so it can easily be invariant over the time. 
This is closely related to discount factors, however no-prior work change discount factors dynamically.
Discounting $Q$ is quite common, and it was present in the initial paper on the $Q$-learning
\cite{watkins1992q}.



% Generalization.
The high-sample complexity, and memorization cannot be easily distinguished
by looking into performance on the test data that has the same distribution 
as the training data. However, it can be verified by 
measuring performance far from the training distribution. 
It's common that researchers
verify performance of their model with slightly more complicated 
test distribution. For instance, speech recognition on longer acoustic
sequences \cite{chorowski2015attention}, 
or machine translation performance parametrized with length of input sequence 
\cite{sutskever2014sequence}. This paper verifies performance of the model
on sequences $100$ times longer than one present during training.










==> old2/rl_expr.tex <==
\section{Reinforcement Learning Experiments}
\label{sec:expr}

Some problems are much easier to solve with stateless models like feed-forward network, 
and are way harder to solve with non-stateless one (especially in setting when actions ). 
The reverse task is an instance of such problem.
Subsection \ref{subsec:expr_generalization} shows how much more difficult it is to solve 
this task with RNNs over FF network.
We report results on all tasks using RNN such as GRU, except of reverse on which we use FF network.
It's quite unsatisfying that we were not able to solve all tasks using the same model.








First, we asses quality of derived models by looking how far
beyond training distribution they generalize. Next, Subsection \ref{sec:dynamic}, \ref{sec:expr_pulled} checks
importance of enhancements that we have proposed in Section \ref{sec:q_learning}.
Subsection \ref{subsec:expr_generalization} analyzes supervised setting, and influence of 
Controller on the final result.


Then, we describe curriculum in Subsection \ref{subsec:curriculum}. 
Finally, we present interesting solutions to the \textit{addition} task that our model found
(Subsection \ref{subsec:multiple_sol}). More experimental results can be found
in the supplementary material.


Reinforcement Learning methods tend to be very non-deterministic, and their performance
highly depends on an initialization seed.
We repeat all of our experiments with $10$ different seeds, and 
budget of processing $3 * 10^7$ characters. Our models process $2000$ characters per sec,
and this constrain corresponds to $250$ min.~walltime.
We provide probability of success in tables, and we depict high values with green color, 
and low one with red.
We count \textit{success} if model solves task with $100\%$ accuracy up to \textit{complexity} 100.
(\textit{complexity} is rough number of steps necessary to solve a problem).
Some of tables consider much harder test dataset (\textit{complexity} up to 1000).
However, then it is clearly stated. Accuracy is measured on a sample basis.
For instance, if task is to reverse sequence $1234$, then
we count as the correct answer only $4321$. Answer like $4344$ would yield $0$ score, even if two first 
predictions are correct. 


Majority of experiments is performed with $200$ unit GRU, batch size of $20$, learning rate of $0.1$, default Glorot 
nitialization multiplied by $2$ (\cite{glorot2010understanding}).
We use some slight curriculum on all our tasks. However, we use an advance one only on 3 rows 
addition task Subsection \ref{subsec:curriculum}.
We inform when there is any departure from this default setting.
Model sees the current input from all interfaces, and last taken action.
We have to provide last taken action, as we sample actions from a policy. 
Only \textit{reverse} task
is trained with a different Controller, which is feed forward network (explanation in Subsection \ref{sec:infty}). 
However, Subsection \ref{subsec:expr_generalization} presents performance with different \textit{controllers} as well.


We refer to our full learning setting as enhanced $Q$-learning. Enhanced $Q$-learning is Watkins's $Q(\lambda)$ with
dynamic discount, and delayed penalty on $Q(s, \bullet)$.



Plots in Figure \ref{fig:accuracy} show how well model generalizes to longer sequences. 
We have repeated all experiments $10$-times. Blue lines correspond to performance
of classical $Q$-learning with no discount, and green lines correspond to 
performance of our enhanced $Q$-learning. Moreover, Table \ref{tab:simple}
compares success rate for $Q$-learning with different discounts.




\input{"experiments/table_simple.tex"}
\hline
\end{tabular}
\caption{Comparison of success rate for classical $Q$-learning versus our enhanced $Q$-learning.}
\label{tab:simple}
\end{table}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.32\linewidth]{generalization/ident.pdf}
  \includegraphics[width=0.32\linewidth]{generalization/reverse.pdf}
  \includegraphics[width=0.32\linewidth]{generalization/addition.pdf}
  \includegraphics[width=0.32\linewidth]{generalization/addition3.pdf}
  \includegraphics[width=0.32\linewidth]{generalization/single_mul.pdf}
  \includegraphics[width=0.2\linewidth]{generalization/legend.png}
  \caption{Plots of test accuracy for all tasks over $10$ runs. Plots are indexed by accuracy over y-axis,
  and complexity over x-axis (in log scale). We count accuracy on a sample basis
  (i.e. single incorrect prediction yields $0$ accuracy for a given sample).
  \textit{complexity} is a rough number of time-steps necessary to solve a task. We index $x$-axis up
  to $2 * 10^4$ time steps. Green area indicates performance of our model with all tricks, and
  blue area performance of classical $Q$-learning.}
  \label{fig:accuracy}
\end{figure}

\subsection{Curriculum Learning}
\label{subsec:curriculum}
XXXX
We choose randomly complexity  of samples starting from the current complexity, which is initially $6$. If model solves given complexity successfully,
and doesn't generalize to complexity $10^3$ then we move to $+4$ complexity. 

Task \textit{3 rows addition} (Figure \ref{fig:tasks}) 
is quite challenging to solve for our model.
We had to employ curriculum learning in order to solve this task. Our curriculum
is almost giving a solution ``on the tray''. For instance, our examples were field with many zeros,
however we were avoid putting zero at the end of sequence. Putting zero at the end of sequence 
could make model agnostic to final character. 
We achieved $\mathbf{80\%}$ success rate with curriculum versus $0\%$ success
rate without.
Samples with curriculum are provided only during training, and
we don't simplify test distribution.
We present examples of samples for \textit{3 rows addition} with Curriculum. The simplest samples are on the
left, and the hardest on the right:
$\mborder{\begin{matrix}1\\ 2\\ 2\end{matrix}}$ ; $\mborder{\begin{matrix}2\\ 0\\ 2\end{matrix}}$ ; $\mborder{\begin{matrix}8 & 3\\ 3 & 3\\ 3 & 7\end{matrix}}$ ; $\mborder{\begin{matrix}3 & 2 & 0 & 6 & 9\\ 1 & 3 & 1 & 3 & 1\\ 2 & 8 & 0 & 8 & 3\end{matrix}}$ ; $\mborder{\begin{matrix}8 & 0 & 1 & 8 & 5 & 2 & 0 & 2 & 1\\ 1 & 3 & 1 & 4 & 0 & 7 & 0 & 5 & 4\\ 3 & 1 & 3 & 2 & 7 & 5 & 0 & 7 & 1\end{matrix}}$.  


\subsection{Time invariant $Q$}
\label{sec:dynamic}
We have introduced time invariant $Q$ in Subsection \ref{subsec:reparametrization}. 
Time invariant $Q$ can be seen as a dynamic discount. That's why we compare this method 
with fixed discounts. 
Table \ref{tab:dynamic} compares results of classical $Q$-learning with $0.95$ discount
and dynamic discount. We have chosen $Q$-learning with $0.95$ discount, because it performed the
best on our tasks among other discounts (Table \label{tab:simple}).


\input{"experiments/table_q_classic.tex"}
\hline

\end{tabular}
\caption{Table presents success rate of classical $Q$-learning with $0.95$ discount, and 
         with dynamic discount.}
\label{tab:dynamic}
\end{table}


\subsection{Watkins's $Q(\lambda)$}
\label{subsec:expr_pulled}
Section \ref{subsec:pulled} describes Watkins's $Q(\lambda)$. This section analyzes its
importance.
We gradually add tweaks to our learning method, so current comparison includes dynamic discount. 
Table \ref{tab:pulled} presents importance of Watkins's $Q(\lambda)$ on our task. 


\input{"experiments/table_q_pulled.tex"}
\hline
\end{tabular}
\caption{Table compares success rate of $Q$-learning with dynamic discount to Watkins's $Q(\lambda)$ with dynamic discount.}
\label{tab:pulled}
\end{table}

\subsubsection{Penalty on $Q(s, \bullet)$}
\label{ref:subsubsec_penalty}
Table \ref{tab:contrastive} compares success rate 
of Watkins's $Q(\lambda)$ with dynamic discount with 
and without penalty on $Q(s, \bullet)$. Results 
are quite consistent when we test on problems with
complexity $100$, as well as $1000$.

\input{"experiments/table_contrastive.tex"}
\caption{Table shows success rate of Watkins's $Q(\lambda$ with and 
without penalty on $Q(s, \bullet)$. Table concerns sequences of length (Left) $100$ and (Right) $1000$.}
\label{tab:contrastive}
\end{table}



\subsection{Solutions to the \textit{addition} problem}
\label{subsec:multiple_sol}
The model finds various correct solutions to \textit{addition} problem (Figure \ref{fig:addition_solutions}).
This finding was suprised for us, as we anticipated only a single solution.
Change in seed or model architecture influences choice of the final solution.


\begin{figure}[h]
  \begin{center}
    \begin{picture}(280, 100)
      \multiput(0,50)(20,0){3}{
        \put(0, 0){\framebox(20, 20){}}
        \put(0, 20){\framebox(20, 20){}}
        \put(20, 0){\framebox(20, 20){}}
        \put(20, 20){\framebox(20, 20){}}

        \put(34, 30){\vector(-0.2, -1){4}}
        \put(29, 10){\vector(-0.2, 1){4}}
        \put(25, 30){\vector(-1, 0){12}}
      }
      \multiput(100, 50)(20,0){3}{
        \put(0, 0){\framebox(20, 20){}}
        \put(0, 20){\framebox(20, 20){}}
        \put(20, 0){\framebox(20, 20){}}
        \put(20, 20){\framebox(20, 20){}}

        \put(29, 30){\vector(-0.2, -1){4}}
        \put(14, 10){\vector(-0.2, 1){4}}
        \put(25, 10){\vector(-1, 0){12}}
      }
      \multiput(200, 50)(40,0){2}{
        \put(0, 0){\framebox(20, 20){}}
        \put(0, 20){\framebox(20, 20){}}
        \put(20, 0){\framebox(20, 20){}}
        \put(20, 20){\framebox(20, 20){}}

        \put(30, 30){\vector(0, -1){20}}
        \put(30, 10){\vector(-1, 0){20}}
        \put(10, 10){\vector(0, 1){20}}
        \put(10, 30){\vector(-1, 0){20}}
      }
    \end{picture}
  \end{center}

  \caption{Our model found several different solutions to the \textit{addition} problem. 
           Figure depicts sequence of read locations over Input Grid. 
           All of discovered sequences allow to properly solve addition task.}
  \label{fig:addition_solutions}
\end{figure}


==> old2/supervised.tex <==
\section{Out of training set generalization}
\label{sec:infty}
The algorithmic tasks
like multi-digit addition, reverse, coping and single digit multiplication 
have deterministic solution
that can be expressed as a simple computer program or even a finite state automata. Such solution yields
$100\%$ accuracy on an arbitrary length sequences. 
We examine if and when neural network can learn
solution that generalizes to much longer lengths with $100\%$ accuracy. 



Consecutive time-steps of the model execution have to 
correspond to the underlaying arithmetic logic of the problem. 
However, there is often no one-to-one mapping. For instance, addition 
as an operation in arithmetic logic involves
(1) bit-wise addition of numbers, (2) alternation of
result by carry, (3) storing carry in register, (4) shifting by one in memory address.
(1, 2, 3) are executed all together internally by the Controller, while (4) is a part
of the action space.





The state of a neural network is completely determined by hidden state vector 
on any layer of hierarchy. For instance, if two different inputs give the same activations
on the first layer, then they would have the same activations on the second layer, and 
further layers.


Ensuring that the state of a network during test matches the state of the network during training
guarantees generalization. It's enough to verify this property for the representation on any layer.
We examine how state of the Controller looks 
for a feed forward network, a feed forward network over few time steps, and 
a recurrent neural network (Figure \ref{fig:state}).



\textbf{A recurrent neural network} iteratively consumes a hidden state $h_t$ and produces 
the new hidden state $h_{t + 1} = f(x_t, h_t)$, where $x_t$ is the input.
The hidden state $h_{t + 1}$ is the result of $t$ applications of the function $f$. 
Function $f$ has to keep an exact orbit over known states in order to hold generalization. 
However, we observe that RNNs 
fail to generalize on sufficiently long sequences (Section \ref{subsec:expr_generalization}).


Moreover, RNN tends to learn transition probabilities on top of the deterministic pattern.
Let's assume that the task is to reverse a sequence (Section \ref{sec:tasks}).
The training data consists of short sequences to reverse, for instance up to $10$ digits.
The model learns that after $10$ digits is should expect the end-of-sequence character.
Figure \ref{fig:automata} presents what automata corresponds to solving reverse problem, 
and what automata RNN learns for short sequences.


            
\begin{figure}[h]
  \begin{minipage}[c]{0.48\linewidth}
    \centering
    \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=2.1cm,scale=0.5, every node/.style={scale=0.55}]
      \node[state] (A)      {{Go right}};
      \node[state]         (B) [right of=A]  {{Go left}};
      \path[->] (A)  edge [loop above] node {} (A)
                     edge              node {} (B) 
                (B)  edge [loop above] node {} (B);
    \end{tikzpicture}
  \end{minipage}
  \hfill
  \begin{minipage}[c]{0.48\linewidth}
    \centering
    \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=2.1cm,scale=0.5, every node/.style={scale=0.55}]
      \node[state] (A0)                {{Go right{\Large $_1$}}};
      \node[state]           (A1) [below of=A0]  {{Go right{\Large $_2$}}};
      \node[state]           (A2) [below of=A1]  {{Go right{\Large $_3$}}};
      \node[state]           (B)  [right of=A0]  {{Go left}};
      \path[->]  (A0) edge              node {} (B)  
                      edge              node {} (A1)
                 (A1) edge              node {} (B) 
                      edge              node {} (A2)
                 (A2) edge              node {} (B) 
                 (B)  edge [loop above] node {} (B);
    \end{tikzpicture}
  \end{minipage}

  \caption{\textbf{(Left)} The automata describing the correct solution to the reverse problem 
  The model first has to go the right while suppressing prediction. Then, it has to go to the left and predict what it sees at the given moment.
  This figure illustrates only actions over the Input Tape. 
\textbf{(Right)} This is an automata to solve \textit{reverse} problem for short sequences. It doesn't generalize to an arbitrary length sequences. Expressive models like RNN tent to learn such incorrect automata.}
  \label{fig:automata} 
\end{figure}




\textbf{A feed-forward network} has no-recurrent connections, so 
it acts the same way regardless of the past states.
Such model is quite weak, as it can solve
problems that doesn't have any time dependency. However, for problems that it can
solve, it generalizes to an arbitrary length, as the state for the short sequences look the same 
as the state for the long one.





\textbf{A feed-forward network over few last time-steps} is a 
feed-forward network that takes several recent time-steps into account.
This model is slightly more powerful than the feed-forward network
over a single time-step. For instance, it can learn to repeat short sequences, which wouldn't 
be feasible for a feed-forward network over single time-step. However, such model cannot solve tasks that
require long distance dependency, like to remember to close a bracket. 


A feed-forward network, or a feed-forward network over few last time-steps 
don't keep a state over the time. This property ensures generalization. 
We call such models \textit{stateless}. The next Section \ref{subsec:expr_generalization} 
experimentally compares generalization when controller is stateless versus when it's not.




\begin{figure}
  \begin{center}
  \begin{minipage}[t]{0.28\linewidth}
    \centering
    \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=1.9cm,scale=0.5, every node/.style={scale=0.55}]
      \node[state]         (S1)     {\large $h_{t - 3}$};
      \node[]         (X1) [below of=S1] {\Large $x_{t-1}$};
      \node[state]         (S2) [right of=S1] {\large $h_{t - 2}$};
      \node[]         (X2) [below of=S2] {\Large $x_{t-2}$};
      \node[state]         (S3) [right of=S2] {\large $h_{t - 1}$};
      \node[]         (X3) [below of=S3] {\Large $x_{t-1}$};
      \node[state, fill=green, accepting]         (S4) [right of=S3] {{\fontsize{20}{20}\selectfont $h_{t}$}};
      \node[]         (X4) [below of=S4] {\Large $x_{t}$};
      \path[->] (X1)  edge node {} (S1)
                (X2)  edge node {} (S2)
                (X3)  edge node {} (S3)
                (X4)  edge node {} (S4);
    \end{tikzpicture}


    Feed forward
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.28\linewidth}
    \centering
    \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=1.9cm,scale=0.5, every node/.style={scale=0.55}]
      \node[state]         (S1)     {\large $h_{t - 3}$};
      \node[]         (X1) [below of=S1] {\Large $x_{t-1}$};
      \node[state, fill=green]         (S2) [right of=S1] {\large $h_{t - 2}$};
      \node[]         (X2) [below of=S2] {\Large $x_{t-2}$};
      \node[state, fill=green]         (S3) [right of=S2] {\large $h_{t - 1}$};
      \node[]         (X3) [below of=S3] {\Large $x_{t-1}$};
      \node[state, fill=green, accepting]         (S4) [right of=S3] {{\fontsize{20}{20}\selectfont $h_{t}$}};
      \node[]         (X4) [below of=S4] {\Large $x_{t}$};
      \path[->] (X1)  edge node {} (S1)
                (S2)  edge node {} (S3)
                (X2)  edge node {} (S2)
                (S3)  edge node {} (S4)
                (X3)  edge node {} (S3)
                (X4)  edge node {} (S4);
    \end{tikzpicture}

    Feed forward network\\
    over few time-steps
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.28\linewidth}
    \centering
    \begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=1.9cm,scale=0.5, every node/.style={scale=0.55}]
      \node[]         (S0)      {};
      \node[state, fill=green]         (S1) [right of=S0]      {\large $h_{t - 3}$};
      \node[]         (X1) [below of=S1] {\Large $x_{t-1}$};
      \node[state, fill=green]         (S2) [right of=S1] {\large $h_{t - 2}$};
      \node[]         (X2) [below of=S2] {\Large $x_{t-2}$};
      \node[state, fill=green]         (S3) [right of=S2] {\large $h_{t - 1}$};
      \node[]         (X3) [below of=S3] {\Large $x_{t-1}$};
      \node[state, fill=green, accepting]         (S4) [right of=S3] {{\fontsize{20}{20}\selectfont $h_{t}$}};
      \node[]         (X4) [below of=S4] {\Large $x_{t}$};
      \path[->] (S0)  edge node {} (S1)
                (S1)  edge node {} (S2)
                (X1)  edge node {} (S1)
                (S2)  edge node {} (S3)
                (X2)  edge node {} (S2)
                (S3)  edge node {} (S4)
                (X3)  edge node {} (S3)
                (X4)  edge node {} (S4);
    \end{tikzpicture}

    Recurrent Neural Network
  \end{minipage}
  \end{center}
  \caption{Figure presents the dependency of the hidden state $h_t$ for the various Controllers. 
  \textbf{(Left)} For a FF network, the state $h_t$ depends only on the current input $x_t$. 
  \textbf{(Middle)} For a FF that consumes several time-steps, $h_t$ depends on the few last time-steps.
  \textbf{(Right)} $h_t$ for an RNN depends on the all previous states and inputs.}
  \label{fig:state}
\end{figure}


\section{Supervised Experiments}
\label{subsec:expr_generalization}
This section establishes upper bound on the performance of our models. 
We provide supervision on actions, and we measure how well our models generalize (Figure \ref{fig:supervised}).
Further sections, analyze models trained with reinforcement learning when supervision over
actions is not present.



\begin{figure}[h]
  \centering
  \begin{minipage}[t]{0.60\linewidth}
    \centering
    \vspace{0cm}
    \includegraphics[width=0.32\linewidth]{supervised/ident_rnns.pdf}
    \hfill
    \includegraphics[width=0.32\linewidth]{supervised/reverse_rnns.pdf}
    \hfill
    \includegraphics[width=0.32\linewidth]{supervised/addition_rnns.pdf}
    \\
    \includegraphics[width=0.32\linewidth]{supervised/addition3_rnns.pdf}
    \includegraphics[width=0.32\linewidth]{supervised/single_mul_rnns.pdf}
    \\
    LSTM (yellow) or GRU (red) as the Controller
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.39\linewidth}
    \centering
    \vspace{0.95cm}
    \includegraphics[width=0.48\linewidth]{supervised/ident_ff.pdf}
    \hfill
    \includegraphics[width=0.48\linewidth]{supervised/reverse_ff.pdf}
    \\
    Feed Forward network as the Controller (it fails on all the rest tasks)
  \end{minipage}
  \caption{Plots of test accuracy for all tasks with \textbf{supervised} actions over $10$ runs. 
  This setting rules out difficulty in finding policy by explicitly providing it. Figure compares performance
  of different Controllers.
  Plots are indexed by accuracy over y-axis,
  and complexity over x-axis (in log scale). We count accuracy on a sample basis
  (i.e. single incorrect prediction yields $0$ accuracy for a given sample).
  The Complexity is a rough number of time-steps necessary to solve a task. We index $x$-axis up
  to $2 * 10^4$ time steps.}
  \label{fig:supervised}
\end{figure}



Surprisingly, the supervision over actions is not enough to yield generalization to an arbitrary length for
powerful recurrent models. 
Only a feed-forward controller could consequently generalize to an arbitrary length. 
However, such Controller is 
quite limited, and wouldn't be able to solve task that require 
memory like addition (memory of a carry). It's unclear how to build a RNN that
would naturally generalize to an arbitrary length sequences. 



Moreover, we look into autocorrelation of a hidden state for a feed-forward network, a small LSTM (200 units), and a large LSTM (400 units)
on the reverse task (Figure \ref{fig:autocorrelation}). 
Autocorrelation $A$ of states $\{h_i\}_{i=1, \dots, T}$ is defined as:
\begin{align*}
  E = \frac{\sum_{k=1}^T h_k}{T} \\
  A_{i,j} = \frac{\langle h_i - E, h_j - E \rangle}{\frac{\sum_{k=1}^T \langle h_k - E, h_k - E\rangle}{T}}
\end{align*}
The autocorrelation matrices show how hidden states relate to each other over the time.
We have chosen all digits in the reverse task to be the same, so state shouldn't vary over the time.
The adjusting plots outline confidence of actions to \textbf{(Green)} \textit{move(right)}, \textbf{(Red)} \textit{move(left)}.





\begin{table}[h]
\small
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|CDDD|}
\hline 
  & Feed-forward & Small LSTM & Large LSTM \\
\hline 
   Confidence &
   \includegraphics[width=\linewidth]{img/confidence_ff_50.pdf} &
   \includegraphics[width=\linewidth]{img/confidence_small_50.pdf} & 
   \includegraphics[width=\linewidth]{img/confidence_medium_50.pdf} \\
   Autocorrelation &
   \includegraphics[width=\linewidth]{img/autocorrelation_ff_50.png} & 
   \includegraphics[width=\linewidth]{img/autocorrelation_small_50.png} &
   \includegraphics[width=\linewidth]{img/autocorrelation_medium_50.png} \\
\hline 
\end{tabular}
\caption{Figure presents autocorrelation of hidden states for \textbf{(Left)}
feed forward network, \textbf{(Middle)} a small LSTM (200 units), and \textbf{(Right)} a large LSTM (400 units).
  The solution to the reverse task is a two state automata 
(Figure \ref{fig:state}), so the hidden states of a neural network should 
be mapped to states of such an automata that solves the problem.
The autocorrelation matrix clearly has two separate components that correspond to
two states of the automata. Moreover, plots outline confidence on actions \textbf{(Green)} \textit{move(right)},
and \textbf{(Blue)} \textit{move(left)}.}
\label{fig:autocorrelation}
\end{table}


The Feed-forward network is able to learn a sharp transition, and doesn't distinguish 
first step, from the second etc. The small LSTM learns transition probabilities of
states and distinguishes the first step, from the second (the confidence changes). 
Similarly, large LSTM learns transition probabilities. However, it learns transition 
probabilities for many more time steps. 




Stack RNN, NTM had to either cut-off recurrent connections, or to use weak recurrent units. 
This was necessary to avoid learning transition probabilities that prevent generalization.
The Controller that we consider is also relatively small (200 units GRU). 
We think, that learning complicated patterns require large number of parameters.  
However, large number of parameters leads to learning undesired patterns 
like transition probabilities.








==> old2/tasks.tex <==
\section{Tasks}
\label{sec:tasks}
We consider several tasks:
copy, reverse, multi-digit addition, 3~numbers addition, 
and single digit multiplication (Figure \ref{fig:tasks}).
Tasks predefine available Interfaces (Table \ref{tab:available})


\begin{table}[h]
\tiny
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|lccc|}
\hline 
\multicolumn{1}{|l|}{\backslashbox{Task}{Interface}} & Input Tape & Input Grid & Output Tape \\
\hline 
Coping & \yes & \no & \yes \\
Reverse & \yes & \no & \yes \\ 
Addition & \no & \yes & \yes \\
3-number Addition & \no & \yes & \yes \\
Single Digit Multiplication & \no & \yes & \yes \\ 
\hline 
\end{tabular}
\caption{This table marks available Interfaces for a given task. 
The difficulty of a task is dependent on the provided Interfaces. Statement
my model solves addition task without specifying available Interfaces 
is non-informative.}
\label{tab:available}
\end{table}



\textbf{The copy task} is to copy symbols from the Input Tape to the Output Tape.
This task is relatively simple to solve. However, it requires mastering
few skills. The model has to learn correspondence between the input symbols and the output symbols.
Moreover, the model has to always call \textit{move(right)} method of the Input Tape,
and \textit{predict(yes)} on the Output Tape.


\textbf{The reverse task} is to reverse sequence of symbols. 
The model should take a sequence from Input tape starting on the initial location until the special 
character ``r'', reverse it, and write the answer to the Output Tape.
The correct solution is to reach ``r'' by calling \textit{move(right)} multiple times.
Next, the model suppose to call \textit{move(left)}. It should copy symbols that are under Input head to the Output Tape.
The controller should repeat this last steps multiple times.


The reverse task is surprisingly difficult and its success is highly dependent on the Controller choice. 
For instance, the powerful models like LSTM, GRU, medium size RNN tend to memorize
symbols on the way to the right. They never go left, and they reverse order in memory. This
solution is perfect for short sequences of symbols, but it doesn't generalize to the longer sequences (more in Section 
\ref{sec:infty}).

\textbf{The addition task} is to add two multi-digit numbers. The numbers to add are provided
on the Input Grid, and are already aligned vertically. The initial reading location
is the last digit of the first number (i.e. right upper corner). The controller
has to learn to attend consecutive, corresponding pairs of digits over provided pair of numbers.
Moreover, the model has to (1) memorize addition table for digits and (2) discover concept of a carry.
Surprisingly, this task has several equivalent solutions (Subsection \ref{subsec:multiple_sol}).


\textbf{The 3-number addition task} is very similar to the addition task, but it involves adding 
$3$ numbers. It requires learning the same set of skills as the previous tasks. However, this task
is more challenging, as the reward is less frequent. Moreover, the carry takes more values: $0$, $1$ and $2$
instead of $0$ and $1$ for the 2-number addition task.



\textbf{The single digit multiplication}. This task is to multiply a single digit with a long multi-digit number. 
This task has the similar complexity as the addition task. 
However the carry for this task can take more values: $\in [0, 8]$. 


Every task is parametrized by the \textit{Complexity}. The \textit{Complexity} 
is a rough number of time-steps necessary to solve a problem.
For instance, reverting a sequence of length $20$ with 
Input Tape Interface requires $40$ time-steps. $20$ steps to 
reach the end-of-sequence character, and $20$ steps to come back.
This estimate is rough, as problems might have multiple solutions (Subsection \ref{subsec:multiple_sol}).


\begin{figure}
  \centering
  \fbox{
    \begin{minipage}[t]{0.18\linewidth}
      \centering
      \vspace{2mm}
      \includegraphics[height=0.5\linewidth]{stills/ident.png}
      \vspace{2mm}
      {\small{\tiny\\}Copy}
      \vspace{3mm}
    \end{minipage}
  }
  \fbox{
    \begin{minipage}[t]{0.18\linewidth}
      \vspace{2mm}
      \centering
      \includegraphics[height=0.5\linewidth]{stills/reverse.png}
      \vspace{2.5mm}
      {\small{\tiny\\}Reverse}
      \vspace{3mm}
    \end{minipage}
  }
  \fbox{
    \begin{minipage}[t]{0.18\linewidth}
      \vspace{2mm}
      \centering
      \includegraphics[height=0.5\linewidth]{stills/addition.png}
      \vspace{2.5mm}
      {\small{\tiny\\}Addition}
      \vspace{3mm}
    \end{minipage}
  }
  \fbox{
    \begin{minipage}[t]{0.18\linewidth}
      \vspace{2mm}
      \centering
      \includegraphics[height=0.6\linewidth]{stills/addition3.png}
      \vspace{1mm}
      {\small{\tiny\\}3~number\\addition}
      \vspace{1mm}
    \end{minipage}
  }
  \fbox{
    \begin{minipage}[t]{0.18\linewidth}
      \vspace{2mm}
      \centering
      \includegraphics[height=0.5\linewidth]{stills/single_mul.png}
      \vspace{0.5mm}
      {\small{\tiny\\}Single digit\\multiplication}
      \vspace{1mm}
    \end{minipage}
  }
  \caption{Figure presents the initial state for the every tasks. The yellow box indicates the starting position
  of the reading head over the Input Interface.
  The gray characters on the Output Tape symbolize the \textbf{target} symbols. 
  The target symbols for addition, 3~number addition, and single digit multiplication are
  provided in the inverted order. Such order is the natural order in which humans provide answer to aforementioned tasks.}
  \label{fig:tasks}
\end{figure}



